Adaptation of MobileNetV2 for Face Detection on Ultra-Low Power Platform

Designing Deep Neural Networks (DNNs) running on edge hardware remains a challenge. Standard designs have been adopted by the community to facilitate the deployment of Neural Network models. However, not much emphasis is put on adapting the network topology to fit hardware constraints. In this paper, we adapt one of the most widely used architectures for mobile hardware platforms, MobileNetV2, and study the impact of changing its topology and applying post-training quantization. We discuss the impact of the adaptations and the deployment of the model on an embedded hardware platform for face detection.

==> tex/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Over the past years, deep learning researcher put a lot of effort in finding efficient architectures, in order to increase the inference throughput of neural networks and reduce the exploitation costs. This section summarizes some of the techniques used to reduce the energy consumed by the neural network algorithms, both in term of the number of computation and parameters storage costs. This section is split into two parts: the first part presents some operations used to create efficient architectures and discusses several optimization techniques. The second part presents state-of-the-art architectures for Object Detection and Face Detection tasks.

\subsection{Efficient Deep Learning}

\subsubsection{MobileNets}
In 2017, a team of researchers introduced the concept of MobileNets \cite{howard2017mobilenets}: neural networks that make use of \textit{depthwise separable convolutions}, producing light-weight models for embedded applications. The MobileNet framework showed strong results on different use cases, such as Object-Detection, Face Embeddings, and Face Attributes classification tasks. MobileNetV2 \cite{zhu2018mobilenetv2} further improves the state-of-the-art performance of mobile models. The paper describes efficient ways of applying mobile models to object detection and introduces two techniques: \textit{Inverted Residual blocks} and \textit{Linear Bottlenecks}. These modules take low-dimensional compressed representations of features as input and expand it to a high dimension. The results is then filtered with a depthwise convolution, which reduce the number of multiply-accumulate (MAC) operations of a model quadratically.

\subsubsection{ShuffleNet}

ShuffleNet \cite{zhang2018shufflenet} introduces a novel form of group convolutions and depthwise convolutions. Group convolutions were introduced by AlexNet \cite{krizhevsky2012imagenet} to distribute the convolutions on two GPUs. ResNeXt \cite{xie2017aggregated} makes extensive use of group convolutions, but only in the 3x3 convolution layers, which results in pointwise convolutions occupying 93.4\% of the multiplication-adds.

ShuffleNet units take advantage of the channel shuffle operation within the group convolutions.
ShuffleNets and MobileNets are the networks of choice for efficient classification tasks. Table \ref{tab:comparison_mobilenet_shufflenet} summarizes the performance of the different architectures compared to bigger networks such as VGG-16\cite{simonyan2014very} and GoogLeNet\cite{szegedy2015going}. MobileNet and ShuffleNet architecture even outperform those networks on image ImageNet classification tasks, while requiring fewer parameters and less computation.

\subsubsection{Reinforcement Learning for Network Architecture Search}

Finding the optimal architecture for inference might not be an easy task for humans. Therefore, automated techniques for architecture search have been developed in order to explore the architecture space more efficiently. NASNet \cite{zoph2016neural} uses Reinforcement Learning combined with a recurrent neural network to generate convolutional neural networks with skip connections. The generated architectures achieved state of the art results on CIFAR-10 \cite{krizhevsky2009learning} dataset. Other techniques rely on previously validated architecture (ResNet\cite{he2016deep}, Inception\cite{szegedy2015going}) and optimize the number of repetition of the same cell types \cite{cai2018efficient}. Other authors use network architecture search to design task-specific architecture, such as Face Recognition \cite{zhu2019neural}.

Recently, platform-aware reinforcement learning was used to develop MobileNetV3\cite{howard2019searching}. This architecture is optimized to run on particular devices, as the algorithm was trained to make optimal tradeoffs between latency and accuracy. The generated models are optimized for the device they will be running on. Two models are generated: MobileNetV3-Large and MobileNetV3-small, which target high and low resource use cases, respectively. 

A second technique, named \textit{NetAdapt}\cite{yang2018netadapt} enables the fine-tuning of individual layers. At each iteration, the algorithm generates a set of modification of the MobileNetV2 architecture that improves the latency compared to the previous step, by reducing the size of expansion layers or reducing the bottleneck in all blocks that share the same bottleneck size. For each proposed architecture, the weights of the initial architecture are restored and truncated accordingly. The architecture is then trained for $T = 10000$ steps to get a rough estimate of the accuracy. When the desired latency is reached, the architecture is retrained from scratch.

\subsection{Compression Techniques}
Besides optimizing the architecture by reducing the number of operations computed inside the layers, many others techniques have emerged to minimize the size of neural networks by reducing the storage required by the parameters and allow embedding of the architectures in low-resource environments.

\subsubsection{Quantization}
Quantization is a technique that transforms a word into a smaller bits representation. In neural networks, quantization is an efficient and simple way of reducing the size of the model by representing weights and biases in reduced precision words. This method has many advantages \cite{krishnamoorthi2018quantizing}: 

\begin{itemize}
	\item \textbf{Simple}: it can be applied to a wide range of model and uses cases. One can use a floating-point trained model and quantize it to obtain a fixed-point model without much accuracy loss. 
	\item \textbf{Storage Memory}: transforming the model weights into 8 bits integer representation effectively reduce the size needed to store the parameters by 4x, with negligible drop in performance.
	\item \textbf{Working memory}: Quantized models also need less working memory, as intermediate activations need less storage memory, which eventually results in better cache reuse.
	\item \textbf{Faster computations}: Most processors efficiently handle 8 bits integer computations.
	\item \textbf {Power comsumption}: Moving 8-bits words require much less power than moving 32-bits floating-point data.
\end{itemize}

Quantization can be applied during or after training. With quantization aware training, the weights are optimized during the training phase, providing better accuracy than the post-training quantization. The backward pass is computed with simulated quantized weight, resulting in simulated quantized activations. The weights are still represented as floating-point to allow gradient backpropagation and are quantized per model or on a per-layers basis \cite{zhou2018adaptive}. Post-training quantization is simpler to apply and allow more flexibility. Once trained, the weights can be represented in any floating-point or binary format, at the cost of lower accuracy than quantization aware ones. Models can be reduced to match the constraints of the target platform, provided that the elementary operations (addition, multiplications, etc...) can be performed given the format of the weights. 

\paragraph{Q-Format:}
While different quantization schemes are available, some models have been quantized down to ternary \cite{hwang2014fixed} and binary networks \cite{rastegari2016xnor}. In this thesis, we explore a specific type of quantization (Q-Format \cite{oberstar2007fixed}). The reason for this choice is influenced by the target platform that will be presented in the following sections. A Q number is composed of an integer part and a fractional part: Q$m.n$ or Q$n$ represent a number where $m$ bits are used for the integer part, and $n$ bits are used for the fractional part. Such number requires $n+m+1$ bits for storage. The choice of $n$ is a tradeoff between the dynamic and the maximal range of the numbers represented. The conversion between Q numbers and floating-point numbers is defined as follow:

\begin{ceqn}
	\begin{align}
	x_{integer} = \lfloor x_{float} \rfloor*2^{n-1}
	\end{align}
\end{ceqn}

\begin{ceqn}
	\begin{align}
	x_{float} = \frac{x_{integer}}{2^{n-1}}
	\end{align}
\end{ceqn}

where $n$ is the number of bits used for the precision.

\subsubsection{Pruning}

Instead of trying to compress the values of the parameters, one can also try to reduce the number of parameters. Pruning goes back as early as 1990, with the work of LeCun, Denker and Solla \cite{lecun1990optimal} on "Optimal Brain Damages" and Karnin on pruning of neural networks weights during training phase \cite{karnin1990simple}. Pruning removes weights that contribute less to the overall performance of the network. Because these weights do not contribute to the evaluation, the resulting network is smaller and faster. Moreover, removing non-contributing weights results in minimal accuracy loss. Iterative pruning is one of the most popular pruning techniques: at regular interval during training, the weights that are closer to zeros are removed (zeroed). The network continues training until the desired accuracy or sparsity of the weights is reached.

\subsubsection{Weights Sharing, Hashing and Distillation}

Besides being compressed or removed, weights can also be clustered to reduce the size of the parameters. Many techniques have emerged to reduce the number of parameters stored in the network, such as weight sharing and weight clustering. HashedNets \cite{chen2015compressing} cluster the weights and store them uses a low-cost hash function to randomly weights into hash buckets,  with all connections in the same bucket share the same values. Huffman coding might also be used to encode the weights efficiently \cite{han2015deep}. Knowledge distillation \cite{hinton2015distilling, yim2017gift}, a technique that copies the knowledge of a large network into a smaller one, may also be used for minimizing the size of a model. However, these techniques are out-of-scope of the current thesis and are only mentioned as possible improvements.

The techniques presented in this section are not mutually exclusive and can be combined to obtain very efficient networks \cite{han2015deep}. Tradeoffs between accuracy, space and computation costs are described in chapter \ref{chap:results}.


\subsection{State-of-the-art Object Detection}
\label{sec:dl_vision}
Object detection (or object localization) is a computer vision task that keeps research active for decades. Old-school computer vision was based on filtering techniques and very sophisticated methods of classification, per pixel or per region of the image. Nowadays, as many computer vision tasks, Deep Learning is the favorite approach for object detection.  

A common technique in object detection tasks is to use transfer learning, where a first network is trained for classification, and then is cut only to keep the feature extraction part. The features extracted are then passed to a second part (block or second network) which performs bounding box regression and classification. Originally, AlexNet, then VGG-16\cite{simonyan2014very} were used as features extractor.

Fast R-CNN \cite{girshick2015fast} was one of the first Deep Learning architecture to perform object detection. The network is a two-stage detector, composed of two parts: the first part propose a set of regions of interest via ROIPooling and generates ~2000 candidate bounding boxes using selective search. The second part generates the final bounding box by predicting the coordinate on a regression output branch and a class on a Softmax output branch. 

In 2015, ResNet\cite{he2016deep} reached 3.6\% error rate on ILSVRC competition, making it the most performant classification network. Therefore, it is now widely used for the feature extraction part to replace VGG and AlexNet networks. Faster-RCNN\cite{ren2015faster} improved the Fast-RCNN network by replacing the first part of the network (proposal) with a Region Proposal Network (RPN). Furthermore, the AlexNet feature extraction part was replaced by ResNet. The RPN uses 9 prior boxes (3 scales and 3 aspect ratio) to propose the regions of interest in a sliding window fashion. The output is a box confidence score and regression to these 9 bounding boxes. The selected regions of interest are presented to the second network, which,  finally, performs classification and refined regression of these bounding boxes.

\begin{table}[h]
	\centering
	\begin{tabular}{lccc}
		\hlineB{3} \\
		\textbf{Detection Frameworks} & \textbf{Train sets} & \textbf{mAP} & \textbf{FPS} \\ \hline
		Fast R-CNN\cite{girshick2015fast}            & 2007+2012      & 70.0         & 0.5          \\ 
		Faster R-CNN VGG-16\cite{ren2015faster}          & 2007+2012      & 73.3         & 7            \\ 
		Faster R-CNN ResNet\cite{he2016deep}          & 2007+2012      & 76.4         & 5            \\ 
		YOLO                          & 2007+2012      & 63.4         & 45           \\
		SSD300\cite{liu2016ssd}                      & 2007+2012      & 74.3         & 46           \\ 
		SSD500\cite{liu2016ssd}                     & 2007+2012      & 76.8         & 19           \\
		YOLOv2 288x288                & 2007+2012      & 69.0         & 91           \\ 
		YOLOv2 352x352                & 2007+2012      & 73.7         & 81           \\ 
		YOLOv2 416x416                & 2007+2012      & 76.8         & 67           \\ 
		YOLOv2 480x480                & 2007+2012      & 77.8         & 59           \\ 
		YOLOv2 544x544                & 2007+2012      & 78.6         & 40           \\ 
		\hlineB{3}
	\end{tabular}
	\captionsetup{justification=centering}
	\caption[Performance comparison on major architectures]{Performance comparison\cite{YOLO9000} on major architectures on PASCAL VOC 2007.}
	\label{tab:speed_comparison_yolo}
\end{table}

YOLO\cite{redmon2016you}, as opposed to FastRCNN, is a one-stage detection network which does not require a region proposal network. The base technique of YOLO is to divide the input space into a grid of 200 small regions (squares). The output of this neural network is a miniature version of the grid input, where each pixel is responsible for one square of the grid. Therefore, each square of the grid can be considered as a prior bounding box. The output is a map contains the probability of membership (i.e., confidence score) to a prior bounding box, the regression of the corresponding bounding box coordinates (offset from the center cell, width and height), and a Softmax layer predicting the class. YOLO uses VGG-16 as a feature extractor, to which the output block is appended.

Compared to FastRCNN, YOLO was much faster (table \ref{tab:speed_comparison_yolo}), but was also making a lot more localization errors, and had relatively low recall compared to region proposal-based methods\cite{YOLO9000}. The original YOLO is trained on 224x224 images (from the AlexNet feature extractor) and predicts images of size 448x448. In YOLOv2, the authors improved the performance of the network by fine-tuning the network on 448x448 resolutions images for 10 epochs, resulting in 4\% mAP improvement on PASCAL VOC dataset. They also introduced prior bounding boxes in the model, by clustering the box dimensions of the PASCAL VOC and COCO dataset. The output predicts the regression predicts the height width as offsets from the cluster centroid. The offset from the center pixel is predicted using a sigmoid function.

In 2018, RetinaNet\cite{retinanet} outperformed the current detection algorithms by introducing a new loss function : the Focal loss. The paper investigates the problem of class imbalance in dense detectors. The first stage of Fast R-CNN and Faster R-CNN rapidly narrow down the set of candidate bounding boxes, filtering out most of the background samples. In the second part of the network, sample heuristics, such as fixed foreground-to-background ratio (1:3) or hard-example mining is performed to keep positive and negative examples balanced. Oppositely, one-stage detectors must process huge amount of object locations (often ~100K) that densely cover spatial positions, scales and aspect ratios. While some of the sampling heuristics are introduced when computing the loss function, they are inefficient because the training is still dominated by negative samples. The cross-entropy (CE) loss for binary classification is defined as :

\begin{equation}
p_t = \begin{cases}
p & \text{if $y=1$}.\\
\textit{}1-p & \text{otherwise}.
\end{cases}
\hspace{1cm}
\textnormal{and}
\hspace{1cm}
CE(p,y) = CE(p_t) = -log(p_t)
\end{equation}

Sometimes, the CE loss is weighted and written as the $\alpha$-balanced CE loss function, where $\alpha \in [0,1]$ is the weighting factor:

\begin{equation}
a_t = \begin{cases}
\alpha & \text{if $y=1$}.\\
\textit{}1-\alpha & \text{otherwise}.
\end{cases}
\hspace{1cm}
\textnormal{and}
\hspace{1cm}
CE(p,y) = CE(p_t) = -\alpha_t log(p_t)
\end{equation}

As an alternative, the authors propose a dynamically scaled cross-entropy loss function, where the scaling factor decays to zero as the confidence in the correct class increases. Here, $\gamma \in [0,5]$ is the modulating factor :
 
\begin{ceqn}
	\begin{align}
	FL(p,y) = -\alpha_t(1-p_t)^\gamma \log(p_t)
	\end{align}
\end{ceqn}

The loss designed to handle extreme imbalance between foreground and background classes during training (e.g., 1:1000). When an sample is misclassified and $p_t$ is small, the modulating factor is near 1 and the loss is unaffected. As $p_t \rightarrow 1$, the factor goes to 0 and the loss for well-classified examples is down-weighted by rate $\gamma$. Typically, the authors use $\gamma=2$,  $\alpha=0.25$ and $p_t=0.9$.

The RetinaNet architecture uses a Feature Pyramid Network (FPN) with ResNet backbone to generate a rich multi-scale convolutional feature pyramid. Two subnetworks are then attached to the backbone to predict the class and one for the regression of the anchor bounding boxes (Figure \ref{retinanet_architecture}). RetinaNet outperforms Faster R-CNN (Table \ref{accuracy_retinanet}) while running at similar speeds (122ms vs 172ms\cite{retinanet} respectively). 

\begin{figure}[h]
	\centering
	\includegraphics[width=15cm]{images/RetinaNet}
	\captionsetup{justification=centering}
	\caption[RetinaNet architecture]{RetinaNet architecture\cite{retinanet}. The network is a one-stage detector that uses a Feature Pyramid Network on top of ResNet. The output of the FPN is fed to two subnetworks for classification and box regression.}
	\label{retinanet_architecture}
\end{figure}

\begin{table}[h]
	\centering
	\begin{tabular}{lcc}
		\hlineB{3} \\
		\textbf{Detection Frameworks} & \textbf{Backbone} & \textbf{AP}   \\ \hline
		Faster R-CNN +++\cite{he2016deep}   & ResNet-101-C4     & 34.9          \\ 
		Faster R-CNN w FPN\cite{lin2017feature}     & ResNet-101-FPN    & 36.2          \\ 
		YOLOv2                        & DarkNet-19        & 21.6          \\ 
		SSD513                        & ResNet-101-SSD    & 31.2          \\
		RetinaNet                     & ResNet-101-FPN    & 39.1          \\
		RetinaNet                     & ResNeXt-101-FPN   & \textbf{40.8} \\
		\hlineB{3}
	\end{tabular}
\captionsetup{justification=centering}
\caption[Performance of RetinaNet on COCO]{Object detection results\cite{retinanet} of RetinaNet on COCO test-dev.}
\label{accuracy_retinanet} 
\end{table}
\newpage
\subsection{State-of-the-art Face Detection}

Face detection is an important problem in computer vision. Past methods have been relying on cascade structures and deformable part models (DPM)\cite{yan2014face}. For a long time, the Viola-Jones algorithm \cite{viola2001rapid}, based on a cascade of classifiers, was considered state of the art for face detection tasks. The classifier used a set of filters to detect universal face features, such as nose, eyes and mouth. Because the features were manually computed, the algorithm was not generalizing well. However, this algorithm was very performant even with a small amount of data and had very high execution speed. 

With the rise of Deep Learning, Convolutional Neural Networks have also been applied to the face detection problem, many of which rely on a cascade detection pipeline. Most of them use object detection-like frameworks, which in this case is reduced to a single-class prediction problem (face / non-face).

While face bounding boxes have been used as standard labeling methods for the detection of the faces, Faceness \cite{yang2017faceness} uses facial attribute annotations to detect faces. In their paper, the authors present a method very robust to occlusion. The Faceness network is a two-stage network. The first part is composed of 5 convolutional neural networks with shared weights. The 5 networks contain 7 convolutional layers that produce 1 heatmap, each of which is responsible for detecting one of the 5 following attributes: hair, eye, nose, mouth and beard. Each of the output maps generates a set of candidate faces, which are then combined by with Non-Maximal Suppression (NMS): given a set of generated candidate windows, the windows are ranked according to their "faceness" score. The score of each face region is then computed and averaged. This helps to prune a large number of false positives. The second stage of the Faceness-Net takes the candidate faces, refines the bounding boxes and classifies them as face/non-face. 

\begin{figure}[h]
	\centering
	\includegraphics[width=14cm]{images/Faceness}
	\captionsetup{justification=centering}
	\caption[Faceness architecture]{Faceness architecture\cite{yang2017faceness}. The first stage proposes faces base on 5 attributes. The second stage uses the face proposal to regress the bounding boxes and classify them as face/non-face}
	\label{faceness_architecture}
\end{figure}

Other architectures perform face detection jointly with other tasks, such as landmark detection in \cite{zhang2016joint}. In this paper, 3 different neural networks are used in a cascade fashion: the first one performs early rejection of face and proposes a first set of bounding boxes (P-Net), while the second one performs bounding box regression and refinement (R-Net) of the bounding boxes. Finally, the last network is similar to the second stage, but aim to describe the face in more details by outputting facial landmarks. By jointly training the network for face detection and face alignment (landmark detection), the network performs slightly better than training only for bounding box regressions. 
 
\subsection{TinyFace} 
When somebody looks at a picture, the cues for recognizing a large object in the picture are different from the ones used to find a small object. Object detection algorithms make use of scale-normalized classifiers (scanning windows running on an image pyramid). Training scale-specific classifiers might suffer from a lack of data for individual and inefficiency of running multiple classifiers at test time. The authors of Tiny-Face\cite{hu2017finding} presents a novel approach to face detection. Instead of using multiple classifiers, 3 networks with shared weights are trained for different scales, such that the resulting single-architecture learns the scale-invariant features of the faces. 

\subsubsection{Importance of context} 
Detecting small objects is still challenging for such networks because of the little information contained in the small size object. By running an experiment on human classification, the authors showed that the context is particularly helpful to find small faces (figure \ref{fig:tiny_context}), suggesting that context should be modeled in a scale-variant manner. The features of deeper convolutional layers tend to have larger receptive fields. Interestingly, smaller receptive fields perform better at detecting small faces, while performing poorly at detecting large faces - it is difficult to find large faces from only seeing the tip of the nose. The results of the paper suggest that one can build multitask templates for detectors of different sizes with identical receptive fields, implementing it as a multi-channel heatmap.

\begin{figure}[h]
	\centering
	\includegraphics[width=11cm]{images/context_tinyface}
	\captionsetup{justification=centering}
	\caption[Importance of context to detect a face]{Importance of context to detect a face. Large faces are easily detected by humans when little context is available around, while it is very difficult to detect small faces. Fixed context drastically reduces the error. Pictures taken from \cite{hu2017finding}.}
	\label{fig:tiny_context}
\end{figure}

\subsubsection{Canonical Bounding Boxes}
The authors computed a set of canonical bounding boxes derived by clustering them into 25 different sizes. They trained models of 3 resolutions (0.5x, 1x, 2x interpolation) to predict the corresponding bounding boxes. From the results of figure \ref{fig:tiny_regimes}a, we can observe that for finding large faces (more than 140px in height), we need to build templates at 0.5x resolution; for finding smaller faces (less than 40px in height), we can use templates at 2x the resolution or the original image. For sizes in between, optimal templates should have 1x resolution.

\begin{figure}[H]
	\centering
	\begin{minipage}{0.4\linewidth}
		\centering
		\includegraphics[height=6cm]{images/regimes}
		\label{fig:regimes}
		(a)
	\end{minipage}
	\hspace{1.5cm}
	\begin{minipage}{0.4\linewidth}
		\centering
		\includegraphics[height=6cm]{images/canonical_old}\\
		\label{fig:canonical_boxes}
		(b)
	\end{minipage}
	\captionsetup{justification=centering}
	\caption[Template resolution analysis and anchors]{(a) Template resolution analysis \cite{hu2017finding}. The x-axis is the target object sizes. The y-axis represents the AP at each target size. (b) Set of corresponding canonical (anchor) bounding boxes. The color corresponds to the optimal resolution at which an object of that size is detected.}
	\label{fig:tiny_regimes}
\end{figure}

During inference, 3 different scales of the input image are fed to the network that predicts a template response at every resolution. After applying non-maximum suppression (NMS) at the original resolution, the final detection results are obtained\ref{fig:tiny_arch}. The canonical bounding boxes can be clustered in two groups, as some of them are duplicated : a bounding box that predicts 50x50 faces at 2x resolution is the duplicate of the bounding box responsible of predicting 25x25 faces at 1x the resolution \cite{hu2017finding}. A-type templates (tuned for 40-140px tall faces) are used on the coarse image pyramid (including 2x interpolation), while only run B-type (tuned for less than 20px tall faces) templates on only 2x interpolated images.
\newpage
Tiny-Face represents the state of the art in Face Detection (table \ref{tab:results_tiny_comp}) and will be our starting point for the development of efficient algorithms running on low-power mobile platforms.


\begin{table}[H]
	\centering
	\resizebox{0.63\textwidth}{!}{
	\begin{tabular}{lccc}
		\hlineB{3} \\
		\textbf{Method} & \textbf{Easy} & \textbf{Medium} &\textbf{Hard} \\ \hline
		 
		 ACF\cite{yang2014aggregate} & 0.659& 0.541& 0.273\\
		 Two-stage CNN\cite{yang2016wider} & 0.681& 0.618& 0.323\\
		 Multiscale Cascade CNN\cite{yang2015facial} & 0.691 & 0.634& 0.345 \\
		 Faceness\cite{yang2017faceness} & 0.713& 0.664& 0.424 \\
		 Multitask Cascade CNN\cite{zhang2016joint} & 0.848& 0.825& 0.598\\
		 CMS-RCNN\cite{zhu2017cms} & 0.899& 0.874& 0.624 \\
		 HR-ResNet50\cite{hu2017finding} & 0.907 & 0.890 & 0.802 \\
		 HR-ResNet101\cite{hu2017finding} &\textbf{0.919} & \textbf{0.908} & \textbf{0.823} \\
		\hlineB{3}
	\end{tabular}
	}
	\captionsetup{justification=centering}
	\caption[Comparison of face detection methods]{Comparison of face detection methods on the WIDER FACE\cite{yang2016wider} evaluation dataset. Table taken from \cite{hu2017finding}.}
	\label{tab:results_tiny_comp} 
\end{table}

\begin{figure}[H]
	\centering
	\includegraphics[width=15cm]{images/tiny_arch}
	%\captionsetup{justification=centering}
	\caption[Detection pipeline of the Tiny-Face network]{Overview of the Tiny-Face network. Source : Tiny-Face paper \cite{hu2017finding}.}
	\label{fig:tiny_arch}
\end{figure}

%% SECTION ABOUT EMBEDDED SYSTEMS
%\section{Deep Learning on embedded devices}
%\subsection{DroneNet}
%\subsection{[OTHER]}

==> tex/setup.tex <==
\section{Setup}
\label{sec:setup}
